Adaptive Attention-Based Model for 5G Radio-based Outdoor Localization

Radio-based localization in dynamic environments, such as urban and vehicular settings, requires systems that efficiently adapt to varying signal conditions and environmental changes. Factors like multipath interference and obstructions introduce different levels of complexity that affect the accuracy of the localization. Although generalized models offer broad applicability, they often struggle to capture the nuances of specific environments, leading to suboptimal performance in real-world deployments. In contrast, specialized models can be tailored to particular conditions, enabling more precise localization by effectively handling domain-specific variations, which also results in reduced execution time and smaller model size. However, deploying multiple specialized models requires an efficient mechanism to select the most appropriate one for a given scenario. In this work, we develop an adaptive localization framework that combines shallow attention-based models with a router/switching mechanism based on a single-layer perceptron. This enables seamless transitions between specialized localization models optimized for different conditions, balancing accuracy and computational complexity. We design three low-complex models tailored for distinct scenarios, and a router that dynamically selects the most suitable model based on real-time input characteristics. The proposed framework is validated using real-world vehicle localization data collected from a massive MIMO base station and compared to more general models.

==> commented.tex <==

% Radio-based localization in dynamic environments, such as urban and vehicular settings, requires models that can efficiently adapt to varying signal propagation conditions, including line-of-sight (LoS), non-line-of-sight (NLoS), and mixed scenarios. In this work, we develop an adaptive localization framework that combines a shallow encoder-only attention model with a switching mechanism based on a single-layer perceptron (SLP). This enables seamless transitions between specialized localization models optimized for different conditions, balancing accuracy, computational efficiency, and reliability. We design three low-complexity localization models tailored for distinct scenarios, prioritizing execution time (measured in clock cycles), model size, and robustness to environmental variations. The SLP-based switching module dynamically selects the most suitable model based on real-time input features, ensuring optimal performance without unnecessary computational overhead. Unlike generalized models, which struggle to capture domain-specific variations, our approach leverages specialized models that efficiently handle diverse propagation characteristics. The framework is validated using real-world measurement data from a commercial base station and a mobile vehicle, demonstrating its ability to adapt in real time while maintaining high localization accuracy. By integrating adaptive computation and hardware-aware optimizations, our method significantly improves positioning performance for applications such as autonomous systems and next-generation wireless networks.
% Specialized models often achieve better performance compared to general models, making them particularly valuable for applications like autonomous systems that need to operate reliably across diverse conditions. Specialized models can capture domain-specific variations and noise patterns more effectively. Generalized models offer broader applicability but often at the cost of efficiency and accuracy. We implement specialized models that can automatically switch between different environments seamlessly, and also tailored to achieve minimum localization error and computational efficiency. Experts of sight: radio based localization using attention based models. Adaptive computation. Adaptive hardware to cope with different scenarios of the environment (LoS, NLoS and mixed). Seamless switching between environments. Encoder only model.
